GraspNet: A Large-Scale Clustered and Densely Annotated Dataset for Object Grasping

Object grasping is critical for many applications, which is also a challenging computer vision problem. However, for the clustered scene, current researches suffer from the problems of insufficient training data and the lacking of evaluation benchmarks. In this work, we contribute a large-scale grasp pose detection dataset with a unified evaluation system. Our dataset contains 87,040 RGBD images with over 370 million grasp poses. Meanwhile, our evaluation system directly reports whether a grasping is successful or not by analytic computation, which is able to evaluate any kind of grasp poses without exhausted labeling pose ground-truth. We conduct extensive experiments to show that our dataset and evaluation system can align well with real-world experiments. Our dataset, source code and models will be made publicly available.

==> dataset.tex <==
\input{latex/fig_component_of_dataset.tex}
\section{GraspNet Dataset}
We next describe the main features of our dataset and how we build it.
\subsection{Overview}
Previous grasping dataset either focuses on isolated object~\cite{jiang2011efficient, mahler2017dex, depierre2018jacquard, yan2018learning} or only labels one grasp per scene~\cite{pinto2016supersizing, levine2018learning}. Few datasets consider multi-object-multi-grasp setting and are small in scale~\cite{zhang2018roi, chu2018real} due to the labor of annotation. Moreover, most of the datasets adopt the rectangle based representation~\cite{jiang2011efficient} of grasp pose, which constrains the space for placing the gripper. To overcome these issues, we propose a large-scale dataset in clustered scenario with dense and rich annotations for grasp pose prediction named \emph{GraspNet}. The GraspNet dataset contains 88 daily objects with high quality 3D mesh models. The images are collected from 170 clustered scenes, each contributes 512 RGB-D images captured by two different cameras, resulting 87,040 images in total. For each image, we densely annotate 6-DoF grasp poses by analytic computation of force closure~\cite{nguyen1988constructing}. The grasp poses for each scene varies from 1,500,000 to 2,500,000, and in total our dataset contains over 370 million grasp poses. Besides, we also provide accurate object 6D pose annotations, rectangle based grasp poses, object masks and bounding boxes. Each frame is also associated with a camera pose, thus multi-view point cloud can be easily fused. Fig~\ref{fig:component_of_dataset} illustrates the key components of our dataset.

\subsection{Data Collection}
We select 32 objects that are suitable for grasping from the YCB dataset~\cite{calli2017yale}, 13 adversarial objects from DexNet 2.0~\cite{mahler2017dex} and collects 43 objects of our own to construct our object sets. The objects vary in shape, texture, size and material. Details will be provided in supplementary files. To collect data of clustered scene, we attach the cameras to a robot arm since it can repeat the trajectory precisely and help automatizing the collecting process. Hand-eye calibration is conducted before data collection to obtain accurate camera poses. Considering different quality of depth image will inevitably affect the algorithms, we adopt two popular RGB-D cameras, Intel RealSense 435 and Kinect 4 Azure, to simultaneously capture the scene and provide rich data. For each cluster scene, we randomly pick around 10 objects from our whole set and place them in a clustered manner. The robot arm then moves along a fixed trajectory that covers 256 distinct viewpoints on a quarter sphere. A synchronized image pair from both RGB-D cameras as well as their camera poses will be saved. The detail setting of our data collection process will be provided in supplementary materials. %Fig~\ref{fig:data_collection} shows the setting for our data collection.

%\input{latex/fig_data_collection.tex}


\subsection{Data Annotation}

\input{latex/table_dataset.tex}
\input{latex/fig_grasp_annotation.tex}
\paragraph{6D Pose Annotation} With 87,040 images in total, it would be labor consuming to annotate 6D poses for each frame. Thanks to the camera poses recorded, we only need to annotate 6D poses for the first frame of each scene. The 6D poses will then be propagated to the remaining frames by:
\begin{equation}
    \mathbf{P}_i^j = \mathbf{cam}_i^{-1}\mathbf{cam}_0\mathbf{P}_0^j,
\end{equation}
where $\mathbf{P}_i^j$ is the 6D pose of object $j$ at frame $i$ and $\mathbf{cam}_i$ is the camera pose of frame $i$. Followed by ICP refinement and human checking, we can annotate 6D poses accurately in an efficient manner. Object masks and bounding boxes are also obtained by projecting objects onto the images using 6D poses.
\vspace{-0.1in}
\paragraph{Grasp Pose Annotation} Different from labels in common vision tasks, grasp poses distribute in a large and continuous search space, which brings infinite annotations. Annotating each scene manually would be dramatically labor expensive. Considering all the objects are known, we propose a two stage automated pipeline for grasp pose annotation, which is illustrated in Fig. \ref{fig:annotation}.

First, grasp poses are sampled and annotated for each single object. To achieve that, high quality mesh models are downsampled such that the sampled points (called grasp points) are uniformly distributed in voxel space. For each grasp point, we sample $V$ views uniformly distributed in a spherical space. Grasp candidates are searched in a two dimensional grid $D\times A$, where $D$ is the set of gripper depths and $A$ is the set of in-plane rotation angles. Gripper width is determined accordingly such that no empty grasp or collision occurs. Each grasp candidate will be assigned a confidence score based on the mesh model.

We adopt an analytic computation method to grade each grasp. The force-closure metric~\cite{nguyen1988constructing, ten2017grasp} has been proved effective in grasp evaluation: given a grasp pose, the associated object and a friction coefficient $\mu$, force-closure metric outputs a binary label indicating whether the grasp is antipodal under that coefficient. The result is computed based on physical rules, which is robust. Here we adopt an improved metric described in~\cite{liang2019pointnetgpd}. With $\Delta\mu=0.1$ as interval, we increase $\mu$ gradually from $0.1$ to $1$ step by step until the grasp is antipodal. The grasp with lower friction coefficient $\mu$ has more probability of success. Thus we define our score $s$ as:
\begin{equation}
s = 1.1 - \mu,
\vspace{-0.05in}
\label{eqn:confidence}
\end{equation}
such that $s$ lies in $(0,1)$.

Second, for each scene, we project these grasps to the corresponding objects based on the annotated 6D object poses:
\begin{equation}
\vspace{-0.05in}
\begin{split}
& \mathbf{P}^i = \mathbf{cam_0}\mathbf{P}_0^i,\\
& \mathbb{G}^i_{(w)} = \mathbf{P}^i\cdot \mathbb{G}^i_{(o)}, 
\label{eqn:transform}
\end{split}
\end{equation}
where $\mathbf{P}^i$ is the 6D pose of the $i$-th object in the world frame, $\mathbb{G}^i_{(o)}$ is a set of grasp poses in the object frame and $\mathbb{G}^i_{(w)}$ contains the corresponding poses in the world frame. Besides, collision check is performed to avoid invalid grasps. After these two steps we can generate densely distributed grasp set $\mathbb{G}_{(w)}$ for each scene. According to statistics, the ratio of positive and negative labels in our dataset is around 1:2. We conduct real world experiment in Sec.~\ref{sec:exp} using our robot arm and verify that our generated grasp poses can align well with real world grasping.


\subsection{Evaluation}
\paragraph{Dataset Split} For our 170 scenes, we use 100 for training and 70 for testing. Specifically, we further divide our test sets into 3 categories: 30 scenes with seen objects, 30 with unseen but similar objects and 10 for novel objects. We hope that such setting can better evaluate the generalization ability of different methods.
\vspace{-0.15in}
\paragraph{New Metrics}
To evaluate the prediction performance of grasp pose, previous methods adopt the rectangle metric that consider a grasp as correct if: i) the rotation error is less than 30$^{\circ}$ and ii) the rectangle IOU is larger than 0.25.

There are several drawbacks of such metric. Firstly, it can only evaluate rectangle representation of grasp pose. Secondly, the error tolerance is set rather high since the groundtruth annotations are not exhaustive. It might overestimate the performance of grasping algorithm. Currently, the Cornell dataset~\cite{jiang2011efficient} has achieved over 99\% accuracy. In this work, we adopt an online evaluation algorithm to evaluate the grasp accuracy. 

We first illustrate how we classify whether a single grasp pose is true positive. For each predicted grasp pose $\mathbf{\hat{P}}_i$, we associate it with the target object by checking the point cloud inside the gripper. Then, similar to the process of generating grasp annotation, we can get a binary label for each grasp pose by force-closure metric, given different $\mu$.

For clustered scene, grasp pose prediction algorithms are expected to predict multiple grasps. Since for grasping, we usually conduct execution after the prediction, the percentage of true positive is more important. Thus, we adopt \emph{Precision@k} as our evaluation metric. $AP$ denotes the average \emph{Precision@k} for $k$ ranges from 1 to 50. Similar to COCO~\cite{coco}, we report $AP$ at different $\mu$. Specifically, we denote \textbf{AP} for $AP$ from $\mu=0.1$ to $\mu=0.5$, with $\Delta\mu= 0.1$ as interval. 

To avoid dominated by similar grasp poses or grasp poses from single object, we run a pose-NMS before evaluation, the details of pose-NMS please refer to supplementary file. 

\if 0
For two grasps $\mathbf{G}_1$ and $\mathbf{G}_2$, we define grasp pose distance $D(\mathbf{G}_1, \mathbf{G}_2)$ as a tuple:
\begin{equation}
    D(\mathbf{G}_1, \mathbf{G}_2) = (d_t(\mathbf{G}_1, \mathbf{G}_2), d_{\alpha}(\mathbf{G}_1, \mathbf{G}_2)),
\end{equation}
where $d_t(\mathbf{G}_1, \mathbf{G}_2)$ and $d_{\alpha}(\mathbf{G}_1, \mathbf{G}_2))$ denote translation distance and rotation distance of two grasps respectively. Let a grasp pose $\mathbf{G}$ be denoted by a translation vector $\mathbf{t}$ and a rotation matrix $\mathbf{R}$, then $d_t(\cdot)$ an $d_{\alpha}(\cdot)$ is defined as:
\begin{equation}
    \begin{split}
        d_t(\mathbf{G}_1, \mathbf{G}_2) &= ||\mathbf{t}_1 - \mathbf{t}_2||,\\
        d_{\alpha}(\mathbf{G}_1, \mathbf{G}_2) &= \arccos \frac{1}{2} (\mathrm{tr}(R_1\cdot R_2^\mathrm{T}) - 1),
    \end{split}
\end{equation}
where $\mathrm{tr}(\mathbf{M})$ denotes the trace of matrix $\mathbf{M}$.

Since translation and rotation are not in the same metric space, we define the NMS threshold as a tuple too. Let $TH = (th_d, th_{\alpha})$, we say $D(\mathbf{G}_1, \mathbf{G}_2) < TH$ if and only if
\begin{equation}
    d_t(\mathbf{G}_1, \mathbf{G}_2) < th_d,\quad d_{\alpha}(\mathbf{G}_1, \mathbf{G}_2) < th_{\alpha}.
\end{equation}

Based on the tuple metric, two grasps are merged when their distance is lower than $TH$. Meanwhile, only the top $K$ grasps from each object are considered according to confidence scores and other grasps are omitted. In evaluation, we set $th_d = 1$ cm, $th_{\alpha} = 5$ degree and $K = 10$.
\fi

\subsection{Discussion}\label{subsec:dataset_discussion}

We compare our datasets with other publicly available grasp datasets. Table~\ref{table_1} summaries the main differences at several aspects. We can see that our dataset is much larger in scale and diversity. With our two-step annotation pipeline, we are able to collect real images with dense annotations, with leverage the advantages from both sides.

For grasp pose evaluation, due to the continuity in grasping space, there are in fact infinite feasible grasp poses. The previous method that pre-computed ground truth for evaluating grasping, no matter collected by human annotation~\cite{jiang2011efficient} or simulation~\cite{depierre2018jacquard}, cannot cover all feasible solution. In contrast, we do not pre-compute labels for the test set, but directly evaluate them by calculating the quality score using force closure metric~\cite{nguyen1988constructing}. Such evaluation method does not assume the representation of the grasp pose, thus is general in practice. Related APIs will be made publicly available to facilitate the research in this area. 

